Entity Tracking via Effective Use of Multi-Task Learning Model and Mention-guided Decoding

Cross-task knowledge transfer via multi-task learning has recently made remarkable progress in general NLP tasks. However, entity tracking on the procedural text has not benefited from such knowledge transfer because of its distinct formulation, i.e., tracking the event flow while following structural constraints. State-of-the-art entity tracking approaches either design complicated model architectures or rely on task-specific pre-training to achieve good results. To this end, we propose MeeT, a Multi-task learning-enabled entity Tracking approach, which utilizes knowledge gained from general domain tasks to improve entity tracking. Specifically, MeeT first fine-tunes T5, a pre-trained multi-task learning model, with entity tracking-specialized QA formats, and then employs our customized decoding strategy to satisfy the structural constraints. MeeT achieves state-of-the-art performances on two popular entity tracking datasets, even though it does not require any task-specific architecture design or pre-training.

==> sections/0_abstract.tex <==

% Fan's version

We present \textbf{\ours{}}, a frustratingly \textbf{S}imple-yet-effective approach for \textbf{E}ntity \textbf{T}racking in procedural text. 
Compared with state-of-the-art entity tracking models that require domain-specific pre-training, \ours{} simply
% \jvj{although we fine-tune simply, but should we mention that designing input/output formats (which could best model the sequence of steps for procedural text) for T5 is not trivial? - since none of the NLP tasks seemed to do that with T5 previously}
fine-tunes off-the-shelf T5 with customized formats and gets comparable or even better performance on multiple datasets.
% \jvj{should we mention a line about how task-specific approaches bring limitations? - say 1) we can't very well utilise knowledge from other NLP datasets; or 2) environmental costs of pre-training; or 3) additional modelling effort. Basically, I feel like we need to motivate why there is need of approaches alternative to task-specific methods} 
Concretely, \ours{} tackles the state and location prediction in entity tracking independently and formulates them as multi-choice and extractive QA problems, respectively. 
Through a series of careful analyses, we show that T5's supervised multi-task learning plays an important role  in the success of \ours{}. 
% Through a series of careful analyses, we show that both T5's supervised multi-task learning and the QA reformulation are important to the success of \simet{}. 
In addition, we reveal that \ours{} has a strong capability of understanding implicit entity transformations, suggesting that multi-task transfer learning should be further explored in future entity tracking research.\footnote{We will release our code and data upon publication.}
% \footnote{Code: \url{https://github.com/iamjanvijay/SET}.}
% indicating a promising direction of reusing T5's great cross-task generalizability for entity tracking.
% We conduct thorough analyses to show such task formats fit T5 the best and that it is the multi-task transfer learning in T5 that leads to superior performance. We further show that \simet{} has demonstrated a great understanding of the implicit entity transformations.




==> sections/1_intro_arxiv.tex <==




Tracking an entity throughout procedural text, such as recipes or scientific processs, is challenging because this task requires a model to understand both surface and underlying dynamics of a process (e.g., Step 2 in Figure~\ref{fig:main_figure} implicitly mentions \textit{water}). 
Recent work on entity tracking can be divided into two lines.
One focuses on designing procedural text-specific fine-tuning architectures as entity tracking models need to make step-wise predictions \cite{gupta-durrett-2019-tracking,tang-etal-2020-understanding-procedural,huang-etal-2021-reasoning,rajaby-faghihi-kordjamshidi-2021-time}. For instance, TSLM \cite{rajaby-faghihi-kordjamshidi-2021-time} introduces time-stamp embeddings into RoBERTa \cite{liu2019roberta} to ensure the model makes a specific prediction for each step of the procedure.
The other line of work focuses on learning better representations for procedural text via domain-specific pre-training \cite{zhang_koala, bai-etal-2021-pre, lemon}. \lemon{} \cite{lemon} achieves great performance by continuing pre-training BART \citep{lewis-etal-2020-bart} on 1 million procedural paragraphs.
Both lines of work effectively move this field forward, but all current solutions are domain-specific and require significant amounts of modeling effort and compute resources.
% \jvj{should we also explicitly mention why these task specific solutions are a limitation? like modelling efforts and identifying domain specific auxilary datasets}
This raises the question of whether entity tracking models can learn from out-of-domain NLP tasks 
% given that this strategy has shown great success in many NLP tasks, such as question answering \citep{khashabi-etal-2020-unifiedqa} and semantic parsing \citep{UnifiedSKG}.
given that cross-task transfer learning has been proven effective for many NLP tasks \citep{vu-etal-2020-exploring}.

In this paper, we present \textbf{\simet{}}, a \textbf{S}imple \textbf{E}ntity \textbf{T}racking approach, which benefits from the latest advances in multi-task transfer learning.
This approach only requires fine-tuning T5 \citep{JMLR:v21:20-074}, which is pre-trained a dozens of NLP tasks and has shown great cross-task generalizability \citep{JMLR:v21:20-074, aribandi2022ext, sanh2022multitask}.
% the product of multi-task learning,
% which has shown great cross-task generalizability in supervised \citep{JMLR:v21:20-074} and zero-shot \citep{sanh2022multitask} settings.
The key idea in this method is to frame entity tracking as tasks that T5 has been pre-trained on and thus facilitate knowledge transfer.
Specifically, we formulate the two sub-tasks of entity tracking, state prediction and location prediction, as multi-choice and extractive QA problems, and then fine-tune T5 on each of them independently. 
Unlike previous methods which make architectural changes to encode the index of the queried step, we simply append the index to the question, like "\textit{What is the location of water in step 2?}", which works well empirically.

As for the results, despite the simplicity of \simet{}, we show that it performs on par or even better than the state-of-the-art methods on both scientific processes (ProPara; \citealp{dalvi-etal-2018-tracking}) and recipes (Recipes; \citealp{Bosselut2017SimulatingAD}).
After a series of thorough analyses, we verify that entity tracking can significantly benefit from the multi-task learning in T5.
In addition, we find that \simet{} can well address the challenge of implicit entity transformations, indicating the necessity of further exploring multi-task transfer learning in future research of entity tracking.

% In all, our contributions are three-fold: 1) We are the first work exploring multi-task learning for entity tracking; 2) Our proposed model \simet{} can rival or outperform state-of-the-art models but only require task-specific fine-tuning; 3) The analysis reveals the potential of multi-task learning in addressing the challenge of implicit entity transformations.
% \fan{Need more thinking.}

\begin{figure*}[!t]
\begin{center}
  \includegraphics[width=0.85\textwidth]{figures/main-cropped.pdf}

\caption{Overview of \simet{} (Simple Entity Tracking). \simet{} is a T5-fine-tuning model, which predicts entity state or location for each step of the procedure in a separate example. State prediction and location prediction are framed as \textbf{multi-choice} and \textbf{extractive} QA problems respectively in \simet{}.
  }
  \label{fig:main_figure}
\end{center}
% \vspace{-15pt}
\end{figure*}

==> sections/5_conclusion.tex <==

We present \simet{}, a simple T5-based fine-tuning approach for entity tracking. 
By reformulating entity tracking to QA problems, \simet{} performs on par or even better than the state-of-the-art in-domain pre-training models.
% By only fine-tuning the off-the-shelf T5 model with our proposed task reformulation, 
% \simet{} achieves nearly the same performance and even better performance than the state-of-the-art without an in-domain pre-training stage. 
Our analyses show that multi-task learning on supervised tasks and QA reformulation is the key of \simet{} achieving good performance as well as understanding challenging implicit entity transformations. 
% We envision that with proper task formats, T5-style multi-task transfer learning can provide great generalization to many novel NLP tasks.

==> sections_old/1_intro.tex <==
Tracking the status of an entity in procedural text, such as recipes or scientific processes, is challenging  because this task requires a model to understand the underlying dynamics of a process (e.g., Step 2 in Figure~\ref{fig:main_figure} implicitly mentions \textit{water}). Earlier work tries to model the entity dynamics throughout the whole process by framing entity tracking as a structured prediction problem~\cite{tandon-etal-2018-reasoning, gupta-durrett-2019-tracking}. 
Recently, pre-trained language models (PLMs) have revolutionized the NLP community, and many papers start to explore task-specific fine-tuning strategies using off-the-shelf PLMs~\cite{gupta-durrett-2019-effective, amini2020procedural, rajaby-faghihi-kordjamshidi-2021-time}. 
As procedural text might be under-represented in those PLMs, more recent work \cite{zhang_koala, lemon} shows that domain-specific pre-training is important for developing a performant entity tracking system. However, these pre-training-based methods are usually compute-intensive, which may lead to significant financial and environmental costs \citep{izsak-etal-2021-train, bai-etal-2021-pre}.

In this paper, we explore a more lightweight solution, which only requires task-specific fine-tuning using T5 \citep{JMLR:v21:20-074}, a language model pre-trained on dozens of NLP tasks and has shown great cross-task generalizability in supervised \citep{JMLR:v21:20-074, aribandi2022ext} and zero-shot \citep{sanh2022multitask} settings.
% the product of multi-task learning,
% which has shown great cross-task generalizability in supervised \citep{JMLR:v21:20-074} and zero-shot \citep{sanh2022multitask} settings.
The key idea in this solution is to frame entity tracking as tasks that T5 has been pre-trained on and design the input/output format properly.
Specifically, we formulate the two sub-tasks of entity tracking, state prediction and location prediction as multi-choice and extractive QA problems, and fine-tune T5 on each of them independently. 
Despite its simplicity, we show that our model performs on par or even better than the state-of-the-art methods on both scientific processes (ProPara; \citealp{dalvi-etal-2018-tracking}) and recipes (Recipes; \citealp{Bosselut2017SimulatingAD}) when using T5-large.
After a series of thorough analyses, we verify that entity tracking significantly benefits from the multi-task learning in T5 and our QA reformulation.
In addition, we reveal that this method can well address the challenge of implicit entity transformations, indicating the necessity of further exploring multi-task transfer learning in future research of entity tracking.

\begin{figure*}[!t]
\begin{center}
  \includegraphics[width=0.85\textwidth]{figures/main-cropped.pdf}

\caption{Overview of \simet{} (Simple Entity Tracking). \simet{} is a T5-fine-tuning model, which predicts entity state or location for each step of the procedure in a separate example. State prediction and location prediction are framed as \textbf{multi-choice} and \textbf{extractive} QA problems respectively in \simet{}.
  }
  \label{fig:main_figure}
\end{center}
% \vspace{-15pt}
\end{figure*}

==> tables/tab-ablation-with-recipes.tex <==
\begin{table}[t!]
% \small
\begin{center}
\setlength{\tabcolsep}{5pt}%Tighter
% \scalebox{0.95}{
\scalebox{0.7}{
\begin{tabular}{lcccccc}

\toprule


% \multirow{2}{*}{\textbf{Target}}
& \multicolumn{ 3}{c}{\textbf{ProPara}}
& \multicolumn{ 3}{c}{\textbf{Recipes}} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7}


& \textbf{Cat-1}
& \textbf{Cat-2}
& \textbf{Cat-3} 
& \textbf{P}
& \textbf{R}
& \textbf{F1} \\

\midrule

\multicolumn{ 7}{c}{\textit{Backbone LM (T5-large size)}} \\

\midrule


T5-v1.1 &	76.2 &	55.6 &	36.2 & 58.8 & 42.7 & 49.5\\
T5-v1.1\textsubscript{\textit{QA-FT}} &	76.9 &	58.4 &	43.7 & 66.1 & 68.8 & 67.4\\
T5 & \textbf{77.3} & \textbf{59.8} &	\textbf{46.0} & \textbf{66.9} & \textbf{70.8} & \textbf{68.8}  \\
% \uqavtwo{} & 76.0 & 58.2 & 40.3  &	77.1 &	59.1 &	43.3\\

% Precision: 66.1, Recall: 68.8, F1: 67.4 T5-v1.1\textsubscript{\textit{QA-FT}}
% Precision: 58.8, Recall: 42.7, F1: 49.5 T5-v1.1

% Cat-1           77.08
% Cat-2           59.13
% Cat-3           43.3

\midrule

\multicolumn{ 7}{c}{\textit{Task Formulation (T5-large)}} \\

\midrule

% Precision: 55.8, Recall: 27.5, F1: 36.8

Process-input & 72.3 & 42.9 &	33.1 & 55.8 & 27.5 & 36.8 \\
Step-input &	76.6 &	57.2 &	41.8 & 66.7 & 64.9 & 65.8 \\
QA (ours) & \textbf{77.3} &	\textbf{59.8} &	\textbf{46.0}  & \textbf{66.9} & \textbf{70.8} & \textbf{68.8} \\

% Step-input
% Precision: 66.7, Recall: 64.9, F1: 65.8

% Cat-1           76.14
% Cat-2           54.73
% Cat-3           41.25

\bottomrule 
\end{tabular}
}
\end{center}
% \vspace{-5pt}
\caption{\label{tab:ablation} 
Top: Comparison of different backbone LMs to investigate the impact of multi-task learning. Bottom: Comparison of different task formulations.
Multi-task learning leads to a better entity tracking model, especially with the QA formulation.
% Ablation studies for \simet{}'s initial checkpoint and I/O format on ProPara and Recipes test-set. QA-Style achieves best performance among the task-formulations. T5 achieves strong performance largely because of being pre-trained on supervised datasets.
}
% \vspace{-15pt}
\end{table}
% \fan{Add ablation on different task formulation.}

==> tables/tab-ablation.tex <==
\begin{table}[t!]
% \small
\begin{center}
\setlength{\tabcolsep}{5pt}%Tighter
% \scalebox{0.95}{
\scalebox{0.8}{
\begin{tabular}{lcccc}

\toprule

&
&\textbf{P}
& \textbf{R}
& \textbf{F1} \\

% \midrule

% \multicolumn{ 4}{c}{\textit{Backbone LM (T5-large size)}} \\

\midrule


\multirow{3}{*}{PLM} & T5-v1.1 &	75.5 &	62.7 &	68.5 \\
 & T5-v1.1\textsubscript{\textit{QA-FT}} &	71.8 &	65.9 &	68.7 \\
& T5 & 73.9 &	68.8 &	71.2  \\
% \uqavtwo{} & 76.0 & 58.2 & 40.3  &	77.1 &	59.1 &	43.3\\




% Precision: 66.1, Recall: 68.8, F1: 67.4 T5-v1.1\textsubscript{\textit{QA-FT}}
% Precision: 58.8, Recall: 42.7, F1: 49.5 T5-v1.1

% Cat-1           77.08
% Cat-2           59.13
% Cat-3           43.3

% \midrule

% \multicolumn{ 7}{c}{\textit{Task Formulation (T5-large)}} \\

\midrule

% Precision: 55.8, Recall: 27.5, F1: 36.8

\multirow{3}{*}{Format} & Process & 90.7 & 26.9 &	41.4  \\
& Step &	76.7 &	57.9 &	66.0  \\
& QA & 73.9 &	68.8 &	71.2  \\


\midrule

% Precision: 55.8, Recall: 27.5, F1: 36.8

\multirow{2}{*}{Size} & Base & 74.8 & 65.1 &	69.6  \\
& Large & 73.9 &	68.8 &	71.2  \\

% Overall Precision 0.748                          
% Overall Recall    0.651                          
% Overall F1        0.696  

\midrule



\multirow{2}{*}{Decoding} & CRF & 73.9 &	68.8 &	71.2  \\
& CRF\textsubscript{bias} & 75.7 &	68.8 &	72.1  \\





% Process Level input
% Overall Precision 0.907                                                                                                                                                                                     
% Overall Recall    0.269                                                                                                                                                                                     
% Overall F1        0.414  

% Step level
% ./document_level_merge_location_state_koala_style_eval.sh propara_eval_files/answers.tsv /nethome/jsingh319/codes
% /pro-text/fan/t5_propara_sentence/test_predictions_372.tsv /nethome/jsingh319/codes/pro-text/fan/t5_propara_sentence_loc_10/test_predictions_245.tsv
% Overall Precision 0.767                                                                                                                                                                                     
% Overall Recall    0.579                                                                                                                                                                                     
% Overall F1        0.660     


% T5-v1.1
% Overall Precision 0.755                          
% Overall Recall    0.627                          
% Overall F1        0.685                          

% T5-v1.1 - finetuning
% Overall Precision 0.718                          
% Overall Recall    0.659                          
% Overall F1        0.687                          

% Final after crf (implicit-explicit)
% -------------------------------------------------
% Overall Precision 0.757                          
% Overall Recall    0.688                          
% Overall F1        0.721                          
% =================================================

% Without implicit explicit.
% -------------------------------------------------
% Overall Precision 0.739                          
% Overall Recall    0.686                          
% Overall F1        0.712                          
% =================================================

\bottomrule 
\end{tabular}
}
\end{center}
% \vspace{-5pt}
\caption{\label{tab:ablation} 
Top: Comparison of different backbone LMs to investigate the impact of multi-task learning. Bottom: Comparison of different task formulations.
Multi-task learning leads to a better entity tracking model, especially with the QA formulation.
% Ablation studies for \simet{}'s initial checkpoint and I/O format on ProPara and Recipes test-set. QA-Style achieves best performance among the task-formulations. T5 achieves strong performance largely because of being pre-trained on supervised datasets.
}
% \vspace{-15pt}
\end{table}
% \fan{Add ablation on different task formulation.}

==> tables/tab-implicit.tex <==
\begin{table}[t!]
% \small
\begin{center}
\setlength{\tabcolsep}{5pt}%Tighter
% \begin{tabular}{l|cc|c|cc}
\scalebox{0.7}{
\begin{tabular}{lcccc}
\toprule

\textbf{Data split}
& \textbf{Model}
& \textbf{Cat-1}
& \textbf{Cat-2}
& \textbf{Cat-3} 
\\

\midrule

\multirow{3}{*}{\textit{all}} & \koala{}  & \textbf{78.5} & 53.3 & 41.3 \\
  % & \simet{}\textsubscript{\tvbase-v1.1}  & 75.7 & 54.9 & 34.6  \\
 & \simet{}\textsubscript{\tvbase{}}  & 76.2 & 59.6 & 42.4  \\
 & \simet{}\textsubscript{\tvlarge{}}  & 77.3 & \textbf{59.8} & \textbf{46.0} \\
 
%  Cat-1           75.69
% Cat-2           54.88
% Cat-3           34.56

\midrule

\multirow{3}{*}{\textit{explicit}} & \koala{}  & \textbf{84.3} & \textbf{76.4} & 49.7 \\
  % & \simet{}\textsubscript{\tvbase-v1.1}  & 80.4 & 66.7 & 44.9  \\
 & \simet{}\textsubscript{\tvbase{}}  & 82.4 & 74.0 & 49.2  \\
 & \simet{}\textsubscript{\tvlarge{}}  & 82.9 & 74.4 & \textbf{52.2} \\

% Cat-1           80.42
% Cat-2           66.68
% Cat-3           44.91

\midrule

\multirow{3}{*}{\textit{implicit}} & \koala{} & 82.4 &	29.8 &	32.0\\
  % & \simet{}\textsubscript{\tvbase-v1.1}  & 82.2 & 39.1 & 31.4  \\
 & \simet{}\textsubscript{\tvbase{}}  & 82.3 & \textbf{42.9} & \textbf{40.0} \\
 & \simet{}\textsubscript{\tvlarge{}} & \textbf{83.1} & 42.7 &	39.9 \\
 
 % Cat-1           82.25
% Cat-2           39.09
% Cat-3           31.45
 

\bottomrule 
\end{tabular}
}
\end{center}
% \vspace{-5pt}
\caption{\label{tab:analysis} Comparison of \koala{} and \simet{} on \textit{implicit} and \textit{explicit} entity transformations via the ProPara test set. Without specifically injecting domain knowledge, \simet{} significantly outperforms \koala{} on the \textit{implicit} subset showing the effectiveness of multi-task learning.}
% \vspace{-15pt}
\end{table}



==> tables/tab-propara-old.tex <==
% *************************************************
% *************************************************
% *************************************************
% merged table for both doc and loc eval
\begin{table*}[t!]
% \small
\begin{center}
\setlength{\tabcolsep}{5pt}%Tighter
% \begin{tabular}{l|cc|c|cc}
\scalebox{0.7}{
\begin{tabular}{lccccccccc}
\toprule

\multirow{2}{*}{ \vspace{-0.3cm} \textbf{Model}}
& \multirow{2}{*}{ \vspace{-0.3cm} \textbf{PLM}} 
& \multicolumn{3}{c}{\textbf{Document-level} }
& \multicolumn{5}{c}{\textbf{Sentence-level} }
\\

\cmidrule(lr){3-5} \cmidrule(lr){6-10}

& 
& \bf{P}
& \bf{R}
& \bf{F1}

& \textbf{Cat-1}
& \textbf{Cat-2}
& \textbf{Cat-3} 
& \bf{macro}
& \bf{micro} 
\\



\midrule

\ncet{} \citep{gupta-durrett-2019-tracking} 

& ELMo

& 67.1
& 58.5
& 62.5

& 73.7
& 47.1
& 41.0
& 53.9
& 54.0 \\

\dynapro{} \citep{amini2020procedural} 
& { BERT\textsubscript{Base}}
& 75.2 
& 58.0 
& 65.5

& 72.4
& 49.3
& \textbf{44.5}
& 55.4 
& 55.5
\\ 

\tslm{} \citetalias{rajaby-faghihi-kordjamshidi-2021-time}
& { RoBERTa\textsubscript{Large}}\textsuperscript{\textdagger}
& 68.4 
& \underline{68.9} 
& 68.6 

& \underline{78.8}
& 56.8	
& 40.9
& 58.8
& 58.4
\\ 
 
\koala{} \citep{zhang_koala}
& { BERT\textsubscript{Base}}\textsuperscript{\textdagger}
& \underline{77.7} 
& 64.4 
& 70.4

& 78.5
& 53.3
& 41.3
& 57.7
& 57.5
 \\ 

\midrule

\multirow{2}{*}{\lemon{} \citep{lemon}}
& { BART\textsubscript{Large}}
& 69.9
& 68.1 
& 69.0 
& 78.8
& 57.2
& 42.9 
& 59.6
& 59.2
\\ 



& { BART\textsubscript{Large}}\textsuperscript{\textdagger}
& 74.8 
& \textbf{69.8}
& \textbf{72.2}
& \textbf{81.7} 
& 58.3
& 43.3 
& \textbf{61.1}
& \textbf{60.7}
\\ 

\midrule

\multirow{2}{*}{\cgli{} \citep{ma-etal-2022-coalescing}}
& { RoBERTa\textsubscript{Large}}\textsuperscript{\textdagger}
& 74.9
& 70.0
& 72.4

& 80.3
& 60.5
& 48.3
& 63.0
& 62.7
\\ 

& { RoBERTa\textsubscript{Large}}\textsuperscript{\textdagger}
& 75.7
& 70.0
& 72.7

& 80.8
& 60.7
& 46.8
& 62.8
& 62.4
\\ 



\midrule

\multirow{2}{*}{\simet{} (ours)}
&  { T5\textsubscript{Base}}  & 73.8 & 64.6 & 68.9 &  76.2	 & \underline{59.6} & 42.4 & 59.4 & 58.8 \\ 


& { T5\textsubscript{Large}} & \textbf{80.2} & 64.5 & \underline{71.5} &  77.3	 & \textbf{59.8} & \textbf{46.0} & \underline{61.0} & \underline{60.6} \\

\bottomrule 
\end{tabular}
 }
\end{center}
% \vspace{-5pt}
\caption{\label{tab:result_propara_merged} 
% Document-level (left) and sentence-level (right) evaluation\footnote{An official leader-board for ProPara document-level evaluation is accessible at: \url{https://leaderboard.allenai.org/propara/submissions/public}} on ProPara dataset. Top-2 models are bold.
Document-level and sentence-level evaluation results on ProPara test set. The best performance is boldfaced, and the second-best performance is underlined.
\textsuperscript{\textdagger} indicates that the language model has been further pre-trained on either in-domain corpus or auxiliary tasks. With T5-large, our \simet{}, a simply fine-tuning method, performs on par with the state-of-the-art model \lemon{}, which requires further pre-training BART\textsubscript{Large} on 1 million procedural paragraphs.
} 
% \vspace{-15pt}
\end{table*}


% *************************************************
% *************************************************
% *************************************************

% \fan{@Janvijay, Add the performance of ET}


==> tables/tab-propara.tex <==
% *************************************************
% *************************************************
% *************************************************
% merged table for both doc and loc eval
\begin{table}[t!]
% \small
\begin{center}
\setlength{\tabcolsep}{5pt}%Tighter
% \begin{tabular}{l|cc|c|cc}
\scalebox{0.65}{
\begin{tabular}{lcccccccc}
\toprule

\multirow{2}{*}{ \vspace{-0.3cm} \textbf{Model}}
& \multicolumn{3}{c}{\textbf{doc-level} }
& \multicolumn{5}{c}{\textbf{sent-level} }
\\

\cmidrule(lr){2-4} \cmidrule(lr){5-9}

& \bf{P}
& \bf{R}
& \bf{F1}

& \textbf{Cat-1}
& \textbf{Cat-2}
& \textbf{Cat-3} 
& \bf{Mac.}
& \bf{Mic.} 
\\



\midrule

% \ncet{} 

% & 67.1
% & 58.5
% & 62.5

% & 73.7
% & 47.1
% & 41.0
% & 53.9
% & 54.0 \\

\dynapro{} 
& 75.2 
& 58.0 
& 65.5

& 72.4
& 49.3
& 44.5
& 55.4 
& 55.5
\\ 

\tslm{}\textsuperscript{\textdagger}
& 68.4 
& 68.9
& 68.6 

& 78.8
& 56.8	
& 40.9
& 58.8
& 58.4
\\ 
 
\koala\textsuperscript{\textdagger}
& \textbf{77.7}
& 64.4 
& 70.4

& 78.5
& 53.3
& 41.3
& 57.7
& 57.5
 \\ 

% \midrule

% \multirow{2}{*}{\lemon{} }
% & 69.9
% & 68.1 
% & 69.0 
% & 78.8
% & 57.2
% & 42.9 
% & 59.6
% & 59.2
% \\ 


\lemon{}\textsuperscript{\textdagger}
& 74.8 
& \underline{69.8}
& \underline{72.2}
& \textbf{81.7} 
& 58.3
& 43.3 
& \underline{61.1}
& 60.7
\\ 

% \midrule

% \multirow{2}{*}{\cgli{}}
% & 74.9
% & 70.0
% & 72.4

% & 80.3
% & 60.5
% & 48.3
% & 63.0
% & 62.7
% \\ 


\cgli{}\textsuperscript{\textdagger}
& \underline{75.7}
& \textbf{70.0}
& \textbf{72.7}

& \underline{80.8}
& \textbf{60.7}
& \underline{46.8}
& \textbf{62.8}
& \underline{62.4}
\\ 



\midrule

% \multirow{2}{*}{\ours{} (ours)}  & 73.8 & 64.6 & 68.9 &  76.2	 & \underline{59.6} & 42.4 & 59.4 & 58.8 \\ 


\textbf{\ours{}} (ours) 
& \underline{75.7} & 68.8 & 72.1
&  76.0	 & \underline{60.0} & \textbf{52.4} & \textbf{62.8} & \textbf{62.6} \\


% Overall Precision 0.757                          
% Overall Recall    0.688                          
% Overall F1        0.721                          

% Cat-1           75.98
% Cat-2           59.94
% Cat-3           52.37
% macro-avg       62.77
% micro-avg       62.61

\bottomrule 
\end{tabular}
 }
\end{center}
% \vspace{-5pt}
\caption{\label{tab:result_propara_merged} Document-level and sentence-level evaluation results on ProPara test set. The best performance is boldfaced, and the second-best performance is underlined. \textsuperscript{\textdagger} indicates that the language model has been further pre-trained on either in-domain corpus or auxiliary tasks. \ours{} performs on par with the prior state-of-the-art models without any pre-finetuning on in-domain corpus.} 


% Document-level (left) and sentence-level (right) evaluation\footnote{An official leader-board for ProPara document-level evaluation is accessible at: \url{https://leaderboard.allenai.org/propara/submissions/public}} on ProPara dataset. Top-2 models are bold.
% Document-level and sentence-level evaluation results on ProPara test set. The best performance is boldfaced, and the second-best performance is underlined.
% \textsuperscript{\textdagger}} indicates that the language model has been further pre-trained on either in-domain corpus or auxiliary tasks. With T5-large, our \ours{}, a simply fine-tuning method, performs on par with the state-of-the-art model \lemon{}, which requires further pre-training BART\textsubscript{Large} on 1 million procedural paragraphs.

% % further pre-training BART\textsubscript{Large} on 1 million procedural paragraphs.


% % \textsuperscript{\textdagger} indicates that the language model has been further pre-trained on either in-domain corpus or auxiliary tasks. With T5-large, our \ours{}, a simply fine-tuning method, performs on par with the state-of-the-art model \lemon{}, which requires further pre-training BART\textsubscript{Large} on 1 million procedural paragraphs.



% \vspace{-15pt}
\end{table}


% *************************************************
% *************************************************
% *************************************************

% \fan{@Janvijay, Add the performance of ET}


==> tables/tab-sentence-propara.tex <==
\begin{table}[t!]
% \small
\begin{center}
\setlength{\tabcolsep}{5pt}%Tighter
% \begin{tabular}{l|cc|c|cc}
\scalebox{0.75}{
\begin{tabular}{lccccc}
\toprule

\textbf{Model}
& \textbf{Cat-1}
& \textbf{Cat-2}
& \textbf{Cat-3} 
& \bf{Mac-Avg}
& \bf{Mic-Avg} 
\\

\midrule

\ncet{} % \citep{gupta-durrett-2019-tracking} 

& 73.7
& 47.1
& 41.0
& 53.9
& 54.0 \\

% \etbert{} % \citep{gupta-durrett-2019-effective} 
% & 73.6 
% & 52.6
% & \NA
% & \NA
% & \NA\\

\dynapro{} % \citep{amini2020procedural} 

& 72.4
& 49.3
& 44.5
& 55.4 
& 55.5
\\ 

\tslm{} % \citetalias{rajaby-faghihi-kordjamshidi-2021-time}

& 78.8
& 56.8	
& 40.9
& 58.8
& 58.4
\\ 
 
\koala{} % \citep{10.1145/3442381.3450126}
& 78.5
& 53.3
& 41.3
& 57.7
& 57.5
 \\ 

% \real{} % \citep{huang-etal-2021-reasoning}

% & 78.4
% & 53.7
% & 42.4 
% & 58.2
% & 57.9\\ 

% \midrule

\lemon{} % \citep{https://doi.org/10.48550/arxiv.2201.08081}


& 81.7 
& 58.3
& 43.3 
& 61.1
& 60.7
\\ 

\hspace{1mm} - w/o pre-training
& 78.8 
& 57.2
& 42.9 
& 59.6
& 59.2

\\ 

\midrule

SET (ours) \\

\hspace{1mm} - \tvbase{} 

&  76.2	 & 59.6 & 42.4 & 59.4 & 58.8 \\ 

\hspace{1mm} - \tvlarge{}
&  77.3	 & 59.8 & 46.0 & 61.0 & 60.6 \\ % crf numbers


\bottomrule 
\end{tabular}
}
\end{center}
\caption{\label{tab:result_propara_sen} Sentence-level evaluation scores for different models on ProPara dataset.}
\end{table}
